The role of the Big Geographic Sort in the circulation of misinformation among U.S. Reddit users

Past research has attributed the online circulation of misinformation to two main factors - individual characteristics (e.g., a person's information literacy) and social media effects (e.g., algorithm-mediated information diffusion) - and has overlooked a third one: the critical mass created by the offline self-segregation of Americans into like-minded geographical regions such as states (a phenomenon called "The Big Sort"). We hypothesized that this latter factor matters for the online spreading of misinformation not least because online interactions, despite having the potential of being global, end up being localized: interaction probability is known to rapidly decay with distance. Upon analysis of more than 8M Reddit comments containing news links spanning four years, from January 2016 to December 2019, we found that Reddit did not work as an "hype machine" for misinformation (as opposed to what previous work reported for other platforms, circulation was not mainly caused by platform-facilitated network effects) but worked as a supply-and-demand system: misinformation news items scaled linearly with the number of users in each state (with a scaling exponent beta=1, and a goodness of fit R2 = 0.95). Furthermore, deviations from such a universal pattern were best explained by state-level personality and cultural factors (R2 = {0.12, 0.39}), rather than socioeconomic conditions (R2 = {0.15, 0.29}) or, as one would expect, political characteristics (R2 ={0.06, 0.21}). Higher-than-expected circulation of any type of news (including reputable news) was found in states characterised by residents who tend to be less diligent in terms of their personality (low in conscientiousness) and by loose cultures understating the importance of adherence to norms (low in cultural tightness).

==> bullets.tex <==
\subsection{Reddit Adoption}
\begin{enumerate}
    \item 
\end{enumerate}

\subsection{Circulation}
\subsubsection{Circulation Volume (news post frequency)}
\begin{enumerate}
    \item We observe that the circulation volume of news (dependent variable) by a given state is highly correlated with the number of Reddit users from that state (independent variable). Indeed, as shown in Figure~\ref{fig:residual}, we see that this single variable is able to explain 95\% of all variance ($R^2\approx 0.95$) we see in circulation volume. 

    \item We then explore additional variables that can explain the remaining residual. Circulation volume residual's correlation (measured using Pearson's Correlation Coefficient) with any given independent variable are shown in Figure~\ref{fig:dv_correlation}.
    \begin{enumerate}
            \item The most positively correlated variables are: i) gdp per capita, ii) population, iii) political engagement, and iv) density (urbanization). In other words, wealthy, urban, and populated states have higher news output, irrespective of news types, than what's expected from their reddit adoption rate. 
            
            \item The most negative correlated variables are: i) cultural tightness, ii) conscientiousness, iii) education (percentage graduated high school) for {\it satire} and {\it reputable} news, and iv) republican. That is, conscientious, republican-leaning states with restrictive social norms have less news output than what's expected of their reddit adoption. The association is more prominent for {\it reputable} and {\it satire} news. For example, the correlation between {\it republican-leaning} and {\it fake} news residual is $-0.27$, but $-0.43$ for {\it reputable} news residual. In other words, users from republican-leaning states are posting considerably less reputable news than what's expected, but less so for fake news.
            
            \item Results for psychological and cultural factors: We see that the variables {\it openness} and {\it neuroticism} are both positively correlated with residual. This observation could be explained by prior research that shows neuroticism is associated with more internet activities. Furthermore, we also see that the remaining 4 variables {\it cultural tightness, extroversion, conscientiousness} and {\it agreeableness} are negative correlated with sharing all news types. The correlations are more prominent for reputable and satire news than fake and lowcred news. In other words, a states' psychological and cultural constraints are more indicative of the state's reputable news output volume than non-reputable news output volume. 
            
            \item Results for socioeconomic factors: We see rich regions have more output for all types of news. The positive correlation is somewhat higher for reputable (0.4) and satire (0.45) news than fake (0.29) and lowcred news (0.35). This could be the result of the population from wealthier states being more politically active (e.g., the correlation between political engagement is gdp is 0.27, see Figure~\ref{fig:statecorr}). Additional, wealth distribution (income gini) doesn't have a strong correlation. \comments{Interestingly, prior results shows that individuals in high socioeconomic classes are more confident in their ability to detect misinformation. Results here does provide some evidence}
        
            \item Results for political factors: states that are more politically engagement have higher output for all news types. The positive correlation is higher for reputable and satire news than fake and lowcred news. This could be the results of more politically engaged states being more knowledgeable thus less likely to propagate misinformation.
            % \item Implications: 
  \end{enumerate}
  \item Next, we use 2 separate regression models for each news type {\it \{reputable, fake, lowcred, satire\}}: i) only including psychological and cultural attributes, and ii) including all state-level attributes. Each model is then fitted using the {\it stepAIC} function in R. Results are summarized in Table~\ref{tab:circulation}.
  \begin{enumerate}
      \item We see that the $R^2$ for {\it psyc fitted} models range from $R^2\approx \{0.2, 0.45\}$. And, the variance explained by psychological and cultural factors is 50\% to 80\% of the variance explained by using all factors for all news. In fact, the regression model using only psychological and cultural factors have a higher adjusted $R^2$ than models that exclusive use socioeconomic ($R^2\approx \{0.1, 0.25\}$) or political factors ($R^2\approx \{0.02, 0.2\}$).

      \item The variables {\it cultural tightness} and {\it conscientiousness} are significant indicators for lower-than-expected circulation for all types of news. Whereas {\it population} is significantly correlated with higher-than-expected circulation even after we account for each state's reddit adoption (total number of reddit users from a state).
      
      \item For models that include all factors, the only variables that are still significant that are also not psychological and cultural factors are {\it population} and {\it no\_highschool} (only for satire news).
  \end{enumerate}
\end{enumerate}

\subsubsection{Return of Investment (ROI)} We explore the proportionality of reputable news v.s. non-reputable news ({\it fake, lowcred, satire}). Conceptually, a state distributes both reputable and non-reputable news. Given a news pool containing {\it reputable} news and nonreputable news ({\it fake, lowcred, satire} or {\it all of the three}). If a state distributes more reputable news proportionately than what's expected of a news pool; then, the state is considered to have a good informational return. In other words, a state's ROI is positive. The formulation of ROI is described in Section~\ref{sec:method}. Further, results are summarized in Table~\ref{tab:roi}.

\begin{enumerate}
    \item The ROI ranges from $\{-3.2\%, 1.6\%\}$, which suggests that states don't deviated significantly from their expected output of reputable v.s. nonreputable news. {\comments{If we switch to cost of investment, the range is more significant $\{-35\%, 105\%\}$}}
    \item ROI is positively correlated with the psychological variable {\it openness} when the news pools are {\it lowcred+reputable} and {\it all news}. 
    \item We also see distinct results for when the news pool is {\it satire+reputable} news. More specifically, percentage of nonwhites is positively correlated with ROI, and density (urbanization) is negative correlated with ROI.
\end{enumerate}

\subsection{Contagion and Influence}

\begin{enumerate}
    \item Geographical contagion is rare on Reddit. As shown on in Figure~\ref{fig:viral1}, 74.8\% of all traditional news articles are only posted by a single author with known geo-location, and 86.7\% by at most 2. The values are comparable for {\it fake, lowcred} and {satire}.  Additionally, only 6.3\% (209.7K) traditional news URLs are shared by 4 or more states. Furthermore, the time gap between the posts are lengthy. As shown in Figure~\ref{fig:viral2}, for all news URLs that reached exactly 5 state, the average cascading time is over a year. This is unsurprising considering that Reddit is functionally an online forum rather than a social media platform. Nevertheless, we still see a significant number of news articles being shared across a wide range of subreddits by users from different states. Specifically, 209.7K traditional news articles are shared by at least 5 states (10\%). The numbers of URLs are 2.23K, 11.0K, 1.14K for {\it fake, lowcred, satire} news respectively. Results here suggest that geographical cascading events are exceeding rare for {\it fake} and {\it satire} news. {\comments{Needs to use all news posts regardless of whether we know the geolocation of the user or not for comparison purposes}}
    \item (influence measured using pagerank): Next, we construct contagion networks of the states using the propagation time-series of the 209.7K traditional news articles and 11.0k lowcred news articles. This process is described in detail in Section~\ref{sec:method}. We then compute states' {\it pagerank} scores separately for the {\it lowcred} and {\it traditional} networks. Finally we examine how a state's psychological, cultural, socioeconomic, and political attributes are associated with the state's pagerank scores. Results are summarized on Table~\ref{tab:pagerank}
    \begin{enumerate}
        \item Focusing on models that only include psychological and cultural factors ({\it psych fitted} ), we see that {\it openness} and {\it extraversion} are both positively correlated with pagerank (or influence) for both {\it lowcred} and {\it traditional} networks. Though, the correlation is more positive for {\it traditional} news.
        \item Focusing on models using all state-level attributes, we see that {\it population} and {\it gdp} are positive indicators, suggesting that populous and urban areas are more influential in distributing both {\it lowcred} and {\it traditional} news. Additionally, we also see that political factors including {\it political engagement} ($\beta=0.062$), {\it swing state}($\beta=0.051$) and {\it republican-leaning}($\beta=-0.094$) are all significantly correlated with a state's pagerank in {\it lowcred} network. In comparison, only {\it swing state}($\beta=0.073$) is significant for traditional network.
    \end{enumerate}
    \item (pagerank differential): Results are summarized on Table~\ref{tab:pagerank_diff}. Interestingly, we see that {\it openness} is the only variable that's significantly correlated with pagerank differential. That is, states with a population that have more flexible thinking (instead of rigid thinking) are more influential in distributing traditional news articles.
    \item (homophily): Finally, we determine whether states of similar attributes are more likely to have a pathway (i.e., edge in the network) for news propagation. Here, we generate assortativity coefficient (described in Section~\ref{sec:method}) for the variables {\it cultural tightness}, {\it ideology} (i.e., republican-leaning), {\it population}, and {\it political} engagement. We see that {\it traditional} and {\it lowcred} news networks are very comparable. Furthermore, the networks tend to be disassortative. That is, dissimilar states are more likely to have a pathway to propagate news articles. Results here significantly differ from states' social network which depicts homophily. \comments{Include assortativity results for {\it openness}}
\end{enumerate}

% Table~\ref{table:influencer} shows that:

% \begin{itemize}
%  \item The construct of cultural tightness-looseness alone explains very little. That is, only 6\% of the variability in influencer score for traditional news, none for satirical news, and only 1\% for low-credibility news, and 1\% for fake news. 


% \item There are other psychological constructs that explain the remaining variability for the four types of news. States that are influencers for traditional news tend to be extroverts, agreeable, culturally  loose, and with a considerable faction of people of color. These factors explain 24\% of the variance.

% \item In a similar vein, states that are influencers for  satirical news tend to be extroverts, agreeable, open to new ideas, and swing states. These factors explain 24\% of the variance.


% \item States that are influencers for  low-credibility news tend to be extroverts, agreeable, open to new ideas, populated, wealthy, and swing states. These factors explain as much as 63\% of the variance of the influencer score.

% \item States that are influencers for  fake news tend to be  emotionally stable, populated, democrats, and  non-swing states. These factors explain 36\% of the variance.
%  \end{itemize}

% \todo{old resutls} Results are summarized in Table~\ref{tab:netinf_contagion}. As shown, population is correlated with higher pagerank for all  news types of misinformation. Additionally, democratic-leaning states have significantly higher pagerank (coef for the variable {\it ideo\_diff} is negative). \todo{dwell on an explanation of the results}


==> diffusion.tex <==
\todo{intro paragraph}
We compared the virality of {\it lowcred}, {\it fake} and {\it satire} articles to that of reputable news. For each types of news, we generate the cumulative fraction of articles that were covered by at least $X$ authors/posts/states/subreddits. As shown in Figure~\ref{fig:viral1}, {\it satire} news articles have a more broader reach than other news articles. Next, we compute the average cascade time for news articles that had different breath of coverage. Results are summarized in Figure~\ref{fig:viral2}. As shown, {\it fake} and {\it satire} articles propagated faster that {\it traditional} news sites when X is low. However, the speech difference is insignificant as X increases. A likely explanation is that misinformation may have more difficulty to reach a broader audience after passing a certain threshold. This observation is consistent with related work~\cite{vosoughi2018spread}.

\begin{figure}[t]
\centering
\begin{subfigure}{0.5\textwidth}
\centering
    \includegraphics[width=0.9\linewidth]{figures/cascade_stats_v2.png}
    \caption{\textbf{Diffusion outreach.} Cumulative fraction of news articles that were covered by X number of posts/authors/states/subreddits [Note, partial data for traditional news]. We see that {\it satire} articles have a broader reach than other shades of news. We also see that {\it fake} and {\it lowcred} articles are comparable to {\it traditional} in breath of reach.}
    \label{fig:viral1}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\centering
    \includegraphics[width=.9\linewidth]{figures/cascade_stats_time_v2.png}
    \caption{\textbf{Diffusion speed.} Average cascading time for news articles that were covered by X number of posts/authors/states/subreddits. We see that {\it satire} and {\it fake} sites tend to take less time on average to reach the same number of states and subreddits than {\it traditional} news.}
    \label{fig:viral2}
\end{subfigure}
\label{fig:virals}
\caption{Diffusion processes for the four types of news on Reddit. (a) Diffusion outreach, and (b) diffusion speed. Satirical news have broader outreach, while fake news are faster to spread.}
\end{figure}


==> influence.tex <==
\subsubsection{Diffusion of news on Reddit}
% \input{diffusion}
\todo{intro paragraph}
We compared the virality of {\it lowcred}, {\it fake} and {\it satire} articles to that of reputable news. For each types of news, we generate the cumulative fraction of articles that were covered by at least $X$ authors/posts/states/subreddits. As shown in Figure~\ref{fig:viral1}, {\it satire} news articles have a more broader reach than other news articles. Next, we compute the average cascade time for news articles that had different breath of coverage. Results are summarized in Figure~\ref{fig:viral2}. As shown, {\it fake} and {\it satire} articles propagated faster that {\it traditional} news sites when X is low. However, the speech difference is insignificant as X increases. A likely explanation is that misinformation may have more difficulty to reach a broader audience after passing a certain threshold. This observation is consistent with related work~\cite{vosoughi2018spread}.

% \begin{figure}[t]
% \centering
% \begin{subfigure}{0.95\textwidth}
% \centering
%     \includegraphics[width=0.9\linewidth]{figures/basic_emo_result.png}
%     \caption{\textbf{Distribution of Emotion}}
%     \label{fig:emo1}
% \end{subfigure}%

% \begin{subfigure}{0.95\textwidth}
% \centering
%     \includegraphics[width=.9\linewidth]{figures/basic_emo_result_v3.png}
%     \caption{\textbf{Distribution of prediction probability for the top 3 most frequently observed emotion.}}
%     \label{fig:emo2}
% \end{subfigure}
% \label{fig:emos}
% \caption{We randomly sample 1K comments for each news type. We then determine the most frequently occurring emotions in Figure~\ref{fig:emo1}. We then review the probability distribution of the top 3 emotions ({\it anxious, hopeful, confident}) in Figure~\ref{fig:emo2} \comments{The highest probability is 0.2, does this mean the model is not a good fit? An additional step here is to sample 1K random comments that are not news related.}.}
% \end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}{0.5\textwidth}
\centering
    \includegraphics[width=0.9\linewidth]{figures/cascade_stats_v2.png}
    \caption{\textbf{Diffusion outreach.} Cumulative fraction of news articles that were covered by X number of posts/authors/states/subreddits [Note, partial data for traditional news]. We see that {\it satire} articles have a broader reach than other shades of news. We also see that {\it fake} and {\it lowcred} articles are comparable to {\it traditional} in breath of reach.}
    \label{fig:viral1}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
\centering
    \includegraphics[width=.9\linewidth]{figures/cascade_stats_time_v2.png}
    \caption{\textbf{Diffusion speed.} Average cascading time for news articles that were covered by X number of posts/authors/states/subreddits. We see that {\it satire} and {\it fake} sites tend to take less time on average to reach the same number of states and subreddits than {\it traditional} news.}
    \label{fig:viral2}
\end{subfigure}
\label{fig:virals}
\caption{Diffusion processes for the four types of news on Reddit. (a) Diffusion outreach, and (b) diffusion speed. Satirical news have broader outreach, while fake news are faster to spread.}
\end{figure}

A sample network generated for {\it lowcred}, denoted as $G_{lowcred}$ is shown in Figure~\ref{fig:lowcred_netinf}. As shown, the node size is proportional to the state's PageRank. Further, darker edge color indicates higher weight. \todo{to be changed} Here, we see that Texas, California, and New York state have the highest prevalence of low-credibility content. They also have the highest number of outgoing and incoming edges. 

\begin{figure}[htb]
\centering
\begin{subfigure}{0.4\textwidth}
\centering
    \includegraphics[width=0.8\linewidth]{figures/netinf_fake_v1_+4_pagerank}
    \caption{{\it Fake} Network}
    \label{}
\end{subfigure}%
\begin{subfigure}{0.4\textwidth}
\centering
    \includegraphics[width=.8\linewidth]{figures/netinf_lowcred_v1_+5_pagerank.png}
    \caption{{\it Lowcred} Network}
    \label{}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\centering
    \includegraphics[width=.8\linewidth]{figures/netinf_satire_+4_pagerank}
    \caption{{\it Satire} Network}
    \label{}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\centering
    \includegraphics[width=.8\linewidth]{figures/netinf_traditional_+5_pagerank.png}
    \caption{{\it Traditional} Network}
    \label{}
\end{subfigure}
\label{fig:networks}
\caption{Networks generated using the 10\% threshold. Nodes are sized and colored according to their pagerank and edge color is proportional to adjusted edge weight.\comments{even with the lowest threshold, we still see that fake and satire have very few connecting edges.}}
\end{figure}

\input{tables/contagion_models}
\input{tables/pagerank_diff_models}
% \input{tables/basic_netinf_top}

\todo{1. what are the correlation between a state's lowcred/fake/satire pagerank and a state's tipping point by  Nate Silver?}
\todo{2. what are the dimensions along which contagion happens? pls put the graphs shown in our previous meetings }
We select the top 5 state-level attributes that are the most correlated with a state's pagerank score: {\it cultural tightness}, {\it population}, {\it ideology}, {\it neuroticism}, and {\it openness}. Here, we measure the homophily of states in the generated networks.

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/basic_netinf_assort_v2}
    \caption{Measuring Network Homophily using Assortativity Coefficients. The boxplots for coefficients are generated using the 10\% and 20\% range. We see that cultural tightness is disassortative mixed for {\it fake} and {\it satire} networks, suggesting that culturally tight states are preferentially attached to culturally loose states.}
    \label{fig:assort}
\end{figure}



==> lagging.tex <==

% %%%%%%%%%%%%
% \newpage
% \subsection{Time-series Lagging}
% In this section, we focus on bursts of misinformation and determining which states are more likely to be the leaders and laggers during these bursts. 

% %number of fake news posts; number of states participating?

% Results are summarized in Table~\ref{tab:lagging}. 


% \input{tables/lagging_stepAIC}
% \subsection{Popularity or Virality}
% \subsection{Content}

% Prior studies on social contagion demonstrates that individuals are more likely to adopt the behaviors of their neighbors\cite{}. In this section, we explore whether states are more likely to post a low-credibility news article if its neighboring states have had posted this article before. Here, we adopt the logistic regression method provided by Hedstrom~\cite{}. Given an specific low-credibility news article $n$ and  state $i$, we apply the following:

% \begin{equation}
% 	\begin{aligned}
% 		L_{it}= a_i + \beta \sum \pi_{ij} * q^{(t-1)}_{j}
% 	\end{aligned}
% \end{equation}
% where:
% \begin{description}
% \item $L_{it}$ is $i$'s log likelihood of initially posting $n$ at time $t$
% \item $\beta$ is the change in state $i$'s propensity to post fake news articles as a result of another state posting them. 
% \item $\pi_{ij}$ is the probability of `contact, or social connectivity between state $i$ and state $j$.
% \item $q^{(t-1)}_j$ is 1, if state $j$ posted $n$ at time $(t-1)$, and is $0$ otherwise. 
% \end{description}

% %, assumed to be a decaying function of the dissimilarity between them (or physical distance between them or social graph distance between them)
% Here , we use 2 separate measures for social connectivity $\pi_{ij}$ i): Jaccard similarity of $S_i$ and $S_j$ where $S_i$ is the set of subreddits that users from $i$ had posted in, and ii) social connectivity index calculated as the total number of times users from $i$ and $j$ and conversed with each other on reddit divided by the product of the number of users from $i$ and $j$ that had posted on reddit.

% We indeed observe a positive $\beta$ value. However, the $R^2$ is very small $<0.0001$, suggesting that the contagion effect explains very little of a state's decision to post a low-credibility news post at a given time.

% %%%%
% \end{comment}
% %%%

% {\lia{Notes for next week}}
% For next week, we will attempt to use graph-based models to determine the impact of social contagion. 



==> note.tex <==
%allcott2017social users are segregated offline, not echo chamber stupid
%As a result, we saw that news circulation on Reddit had not been a function of platform network effects. Instead, a state's news circulation was primarily the result of the absolute number of Reddit users from that state. Moreover, the number of news posts scaled linearly with the number of Reddit users which is likely due to the lack of diffusion. Surprisingly, we also observed that a state's personality and culture were better indicators for the remaining residual than the state's socioeconomic conditions and political characteristics. Specifically, we showed that states ranked low in conscientiousness and cultural tightness were significantly less likely to share news, irrespective of news type.

% We propose the following method to determine state-level attributes that are correlated with the states' overall volume (or output) of the types of news. 



%In this section, we included separate regression models fitted with only socioeconomic variables (Table~\ref{tab:circulation_partial_socio}) or political variables (Table~\ref{tab:circulation_partial_pol}), or all variables except for personality and culture (Table~\ref{tab:circulation_partial_other}). We then compared the $R^2$ of these models with the models fitted with only personality and cultural variables (Table 3 in the main text). We observed that the models fitted with only personality and cultural variables had the highest $R^2$ than models fitted with only socioeconomic or political variables. Additionally, by comparing the full models from Table 3 and models that included all variables except for personality and culture (Table~\ref{tab:circulation_partial_other}),  we also saw that personality and cultural variables explained any additional 10\% to 20\% of the variance in the full models.

% We also included two additional robustness checks for the circulation analysis. We first computed the average number of comments by users from a state that contained URLs of a particular news type. We then adopted Equation~1 (see main text) to determine whether personality and cultural variables remained strong indicators for circulation. Results are summarized on Table~\ref{tab:circulation_ave}. As shown, these variables were still indicative of circulation for all news types.

% Next, given that prior studies had shown that fake and low-credibility news is politically-driven~\cite{vosoughi2018spread}, we ran separate analyses for news circulation on political versus non-political subreddits. More specifically, we obtained a list of 1.4K political subreddits from related work~\cite{rajadesingan2021political}; subreddits not listed were considered non-political. We then computed $Circulation(s,i)$ separately for each type of subreddit. Table~\ref{tab:circulation_pol} and Table~\ref{tab:circulation_nonpol} contain the results, which were comparable with our prior observations. 

% \input{tables/circulation_models_pol}
% \input{tables/circulation_models_nonpol}



==> related.tex <==
Past research focused on the circulation of misinformation can be categorized into 2 sub-fields: i) work that predominantly explored how individual characteristics (e.g., personality and culture, socioeconomic class, and political-leaning) are associated with the individual's tendency to share fake news, and ii) studies on network effects which were centered on the characteristics of online communities (e.g., homophily, network influence, and contagion) associated with the distribution of misinformation. 

For individual characteristics, prior studies focused on the big-5 personality traits showed that conscientious individuals are significantly less likely to read and spread false content, whereas credulous individuals are significantly more likely~\cite{forgas2019social,balestrucci2020credulous}. Additionally, individuals ranked high in agreeableness (prosocial, affectionate), are also less likely to seek out false content organically~\cite{buchanan2019spreading}. Likewise, an individual's cultural upbringing (e.g., religiosity) and accepted social norms are also indicative of their propensity to engage with low credibility or fake news content online~\cite{bonney2018fake,islam2020misinformation}. As an example, past work~\cite{islam2020misinformation} demonstrated that religiosity is positively correlated with the sharing of unverified Covid-19 information on social media. Furthermore, work by Allcott et al.~\cite{allcott2018trends}, Grinberg et al.~\cite{grinberg2018fake}, and Kang et al.~\cite{khan2019recognise} revealed that individual's propensity to share fake news is also mediated by their demographic, socioeconomic, and political background. Specifically, older, conservative-leaning, and less information literate individuals are more likely to spread fake news~\cite{allcott2018trends,grinberg2018fake,khan2019recognise}. Results from subsequent studies were largely congruent with these initial findings~\cite{guess2019less,jones2021does,he2019online}. Moreover, individuals may also spread misinformation without actually believing in its veracity~\cite{arceneaux2021some}. This behavior is moderated by the need for chaos, or the desire to attack ideological opponents~\cite{arceneaux2021some}.

Next, focusing on social surroundings (or networks) of people, work by Pariser~\cite{pariser2011filter}, Jamieson\&Cappella~\cite{jamieson2008echo}, and Aral~\cite{aral2020hype} highlighted that social media platform functionalities had facilitated the formation of small, dense, homophilous, and insulated online communities (often called echo chambers or filter bubbles). These communities had then enabled misinformation to spread far and wide quickly~\cite{vosoughi2018spread,tornberg2018echo,asatani2021dense}. For instance, Cinelli showed that users on Facebook are much more ideologically segregated compared to those on Reddit~\cite{cinelli2021echo}. In addition, users were also observed to be more likely to share ideologically congruent low-credibility news content to their immediate network~\cite{guess2021cracking}. Furthermore, recent work by Asatani~\cite{asatani2021dense} suggested that fake news tends to be first posted within densely connected core nodes (individuals highly active in sharing fake news), and then spread out to peripheral nodes more loosely connected to the core. Results here have eventually led researchers to explore network-based strategies to curtail the diffusion of misinformation~\cite{campan2017fighting}.

More recently, researchers had sought to examine these two types of factors collectively~\cite{shu2019studying,li2020real,baptista2021brave}. For instance, Shu et al.~\cite{shu2019studying} and Hamdi et al.~\cite{hamdi2020hybrid} both adopted an individual's personal characteristics and their network attributes when predicting the individual's likelihood of sharing misinformation. In addition, work by Ahmed~\cite{ahmed_detection_2017} suggested that politically active users with more extensive networks are more likely to share misinformation than those with smaller networks. However, this association does not extend to politically inactive users. 

Unlike these previous studies, our paper is focused on the regional characteristics of U.S. states in association with the states' circulation of both true and false news.


==> rqs.tex <==
\begin{enumerate}
    \item RQ1 (Reddit adoption) which states have a higher adoption of Reddit? What are the state-level attributes indicative of adoption rate?
    \item RQ2 (circulation volume)
        \begin{enumerate}
            \item which states are outputting more reputable or non-reputable news than what's explained by the adoption rate? 
            \item which states have disproportionate output for misinformation? In other words, is a state's circulation volume of misinformation more than what expected?
            \item What are the state-level attributes indicative of circulation ?
        \end{enumerate}
    \item RQ3 influence
        \begin{enuma}
            \item Do we see contagion on Reddit?
            \item 
        \end{enuma}
    % \item [Tentative] RQ (audience breadth or audience reach): which states' outreach are more concentrated? For example, are states mainly posting fake news articles in a concentrated handful of subreddits, or are the posts more spread out across different subreddits \comments{Measured using gini right now}? Which states are reaching more audience than what's expected? For example, are states that are more extroverted more likely to post misinformation across a broad range of different subreddits, thus having a broader audience that an introverted state that only posts on a couple of subreddits? \comments{Maybe we can classify subreddits into {\it misinformation-prone} and {\it generic}, we can then examine whether a state is more often posting on {\it misinformation-prone} subreddits (less likely to experiencing another redditor challenging the comment) or {\it generic} subreddits (more likely to experience challenge from other redditors)}.
    % \item [Tentative] RQ (coverage): which states have more diverse coverage than what's expected? \comments{need to think more about how to measure this.}
\end{enumerate}

==> story.tex <==
\subsection{Version 2}
[SITUATION] Fake news is a major contributor to various contemporary political and social issues in the United States. Indeed, many news media pundits and communication scholars alike have proscribed fake news as a key element that led to wide range of controversies and crises in the United States including i) the Clinton Email and Pizzagate conspiracies in 2016, ii) the immigration crisis (migrant caravans) in 2018, and iii) the January 6th, riot in the U.S. Capitol building in 2021. Alarmed by its continued grip on a significant portion of the U.S. population and persistent negative ramifications, researchers have extensively examined factors associated with an individual’s consumption and spread of misinformation. The aim of such research was to identify characteristics (e.g., personality, cultural identity, political leaning, education, socioeconomic class, or homophily of a social network) that heightened the risk of an individual falling victim to misinformation, and to determine approaches that can best inoculate (e.g., increase information literacy) people against false content. Through comprehensive analysis, prior studies have revealed key psychological and cultural factors of an individual and characteristics of their social surroundings (i.e., social network) that were indicative of their tendency to engage with misinformation\cite{bonney2018fake,forgas2019social,burbach2019shares,giachanou2020role,pennycook2020falls,calvillo2021personality,grinberg2019fake,sindermann2020age}. For example, conscientious (careful, diligent) individuals were shown to be significantly less likely to read and spread false content, and whereas credulous individuals tended to be significantly more likely~\cite{forgas2019social}. Additionally, individuals ranked high in agreeableness (prosocial, affectionate), were also less likely to interact with false content~\cite{buchanan2019spreading}. Likewise, an individual's cultural upbringing (e.g., religiosity) and accepted social norms were also suggestive of their propensity to engage with low credibility or fake news content online~\cite{bonney2018fake}. Focusing on social surroundings (or networks) of people, studies also demonstrated that fake news were often consumed and spread by individuals that were situated within small, dense, homophilous and insulated online communities~\cite{vosoughi2018spread}.

[COMPLICATION] Those were all important contributions to the field of misinformation. Yet, there were several noteworthy caveats. First, many of the studies focused on the psychological dimensions of individuals were done in laboratory setting (e.g., Amazon Mturk surveys)~\cite{pennycook2020falls,calvillo2021personality,sindermann2021evaluation,bronstein2019belief}. Additionally, they were also primarily focused on individual's ability to identify misinformation~\cite{pennycook2020falls,calvillo2021personality,sindermann2021evaluation} rather than sharing (or circulation). Indeed, individuals may choose to (and often do) spread misinformation without actually believing in its veracity~\cite{arceneaux2021some}. Furthermore, studies that were focused on sharing behavior, also tended to focus exclusively on false content~\cite{lawson2020pandemics,burbach2019shares,arceneaux2021some}. For example, work by Lawson and Kakkar~\cite{lawson2020pandemics} highlighted that individuals ranked high in conscientiousness were less likely to share misinformation without assessing whether the same individuals were also less likely to share reputable news in general, and whether they more readily shared fake news over reputable news, or vice versa. Finally, previous studies were dominantly focused on individuals or online communities, and had yet to consider the geographical regions of the United States in relation to the circulation of fake news. To elaborate, many previous work have demonstrated that people's preference to live in regions with like-minded others had resulted in ideological and cultural sorting of states~\cite{bishop2009big,abrams2012big}. The United States consists of ``blue", ``red", and ``swing" state. Further, much like a living entity, each state depicts distinct personality and culture. As an example, work by Rentfrow et al.~\cite{rentfrow2013divided} have shown that Utah and New York state was been the most and least agreeable among all the states respectively. South Carolina was the most conscientious, and Maine the least. Similarly, Mississippi had the most restrictive cultural and social norms, whereas California the most loose~\cite{rentfrow2013divided}. Often times, a handful of states alone can determine critical political outcomes (e.g., the result of the 2016 presidential election was decided by only 80K voters from 3 swing states and the outcome of Georgia's 2020 Senate races yielded the U.S. Senate to the Democrats). As such, how fake news sharing behavior vary between states necessitated a more in-depth analysis. Thus far, however, related work on the geographical circulation of misinformation in particular were surprisingly sparse.

[PROPOSAL] Our paper addressed these aforementioned gaps by exploring the role of personality and culture of U.S. states in the spread of both true and false news. To elaborate, we used a list of reputable and nonreputable news sites aggregated by prior work~\cite{bozarth2020higher}, we assigned them into 4 types: {\it fake, lowcred, satire}, and {\it traditional}. Note that there were 934 {\it fake} news sites, 1801 {\it lowcred} sites, 110 {\it satire} sites, and 8.1K {\it reputable} news sites. We then scrapped Reddit archival data between January, 2016 to December 2019 using \url{pushshift.io}, and collected comments that contained at least 1 URL to a known news site. Next, we obtained the estimated geographical location of 2.5M users from related work~\cite{} and expanded the dataset to 3.0M users using the same process from the related work (see detail in Section~\ref{sec:data}). We observed that 822.5K comments containing news links had been posted by users with an estimated geographical location in one of the 50 U.S. states. Finally, we aggregated 14 state-level attributes from related work~\cite{rentfrow2013divided,howard2018social} and American Community Survey (ACS) where were assigned into 3 categories: i) 6 personality and cultural attributes, ii) 5 socioeconomic characteristics, and iii) 3 political factors.

Through in-depth analysis, our paper provided the following important findings:
\begin{enumerate}
    \item We observed that a state's news circulation volume was dominantly a result of number of users present from that state. In fact, the number of users alone explained 95\% ($R\approx 0.95$) of the variance we saw in circulation volumes across the states. Interesting, the remaining residual can be explained predominantly by personality and cultural factors. More specifically, the variance explained by personality and cultural factors was 50\% to 80\% of the variance explained by using all factors. In fact, the regression model using only psychological and cultural factors had a higher adjusted $R^2$ than models that exclusively used socioeconomic ($R^2\approx \{0.1, 0.25\}$) or political factors ($R^2\approx \{0.02, 0.2\}$). In other words the personality and culture of states were more indicative of news circulation volume than political and socioeconomic factors.
    \item Next, by comparing state's sharing of reputable news v.s. non-reputable news, we observed that states rated high in {\it openness}(imaginative and spontaneous), had significantly higher output of reputable news than average, suggesting that these states had better informational return.
    \item Furthermore, unlike individual-centric social networks where news can easily cascade from one person to another resulting in fast and broad contagions, we observed that news contagion had been rare for states. Our analysis revealed that 86.7\% of all news articles were shared by only 1 or 2 redditors located in one of 50 states. Only 7.3\% or 209.7K of all reputable URLs were eventually posted by users from 5 or more distinct states. The numbers of URLs were 2.23K, 11.0K, 1.14K for {\it fake, lowcred, satire} news respectively, suggesting that contagion was practically nonexistent for {\it satire} and {\it fake} articles. Additionally, even when news cascades did occur, cascading on Reddit took much longer compared to Twitter and Facebook. For the URLs that were posted by at least 5 states, the average cascading time had been more than a year (results are comparable irrespective of news types). Lastly, news propagation was disassortative. In other words, news article diffused from a state to other states that are dissimilar. More surprisingly, we observed that results were similar for both reputable and low-credibility news.
    \item \comments{more analysis}
\end{enumerate}

%
%Further, the electoral college of the United States assures that a handful of battleground states alone can determine critical political outcomes (e.g., the result of the 2016 presidential election was decided by only 80K voters from 3 swing states). Indeed, prior literature has extensively observed that geographical entities exhibit distinct ``personalities" and culture, similar to that of a living entity~\cite{rentfrow2013divided}. As an example, work by Rentfrow et al.~\cite{rentfrow2013divided} shows that Utah and New York state is the most and least agreeable among all the states respectively. South Carolina is the most conscientious, and Maine the least. Similarly,  Mississippi has the most restrictive cultural and social norms, whereas California has the most loose~\cite{rentfrow2013divided}. In our work, we explore the connection between each U.S. state's personality traits, cultural factors, and the state's circulation of true and false news. 









\subsection{Version 1}
Prior studies on misinformation demonstrates that an individual's personality (or psychological constraints), such as credulity, is an significant indicator of their tendency to consume and circulate misinformation~\cite{forgas2019social,burbach2019shares,giachanou2020role,pennycook2020falls}. For instance, conscientious (careful, diligent) individuals are significantly less likely to read and spread false content, and whereas credulous individuals are significantly more likely~\cite{forgas2019social}. Additionally, individuals ranked high in agreeableness (prosocial, affectionate), are also less likely to seek out false content organically~\cite{buchanan2019spreading}. Likewise, an individual's cultural upbringing (e.g., religiosity) and accepted social norms are also indicative of their propensity to engage with low credibility or fake news content online~\cite{bonney2018fake}. 

For our work, we expand the existing literature by exploring the role of personality and culture of U.S. states in the spreading of misinformation. Indeed, prior literature has extensively observed that geographical entities exhibit distinct ``personalities" and culture, similar to that of a living entity~\cite{rentfrow2013divided}. As an example, work by Rentfrow et al.~\cite{rentfrow2013divided} shows that Utah and New York state is the most and least agreeable among all the states respectively. South Carolina is the most conscientious, and Maine the least. Similarly,  Mississippi has the most restrictive cultural and social norms, whereas California has the most loose~\cite{rentfrow2013divided}. In our work, we explore the connection between each U.S. state's personality traits, cultural factors, and the state's circulation of true and false news. This analysis is particularly valuable given that prior studies on misinformation demonstrates that false content in the United State is often politically driven~\cite{lazer2018science}. In additional, the political structure of the United States assures that a handful of battleground states alone can determine critical political outcomes (e.g., the result of 2016 presidential election was decided by only 80K voters from 3 swing states). Given these considerations, understanding the regional differences of misinformation can provide valuable insights into its potential downstream impact. 

In our paper, we focus on the distribution of true and false new on Reddit by users from different U.S. states in relation to the personality and culture of the states. To elaborate, we use a list of reputable and nonreputable news sites aggregated by prior work~\cite{bozarth2020higher}, we assign them into 4 types: {\it fake, lowcred, satire}, and {\it traditional}. We note there are 934 {\it fake} news sites, 1801 {\it lowcred} sites, 110 {\it satire} sites, and 8.1K {\it reputable} news sites. We then scrap Reddit archival data between January, 2016 to December 2019 using \url{pushshift.io}, and collect comments that contain at least 1 URL to a known news site. Next, we obtain the estimated geographical location of 2.5M users from related work~\cite{} and expand the dataset to 3.0M users using the same process from the related work (see detail in Section~\ref{sec:data}). We observe that 822.5K comments contain news links had been posted by users with an estimated geographical location in one of the 50 states. Finally, we aggregate 14 state-level attributes from related work~\cite{rentfrow2013divided,howard2018social} and American Community Survey (ACS) assigned into 3 categories: i) 6 personality and culture attributes, ii) 5 socioeconomic characteristics, and iii) 3 political factors.

Our analysis is divided into 3 parts. First, prior to exploring the role of personality and culture in the geographical characteristics of misinformation, we first evaluate the representativeness of users on Reddit with respect to the population of a state. Indeed, past literature shows that male, younger, and liberal-leaning population is more disproportionately represented on Reddit~\cite{duggan20136}. Here, we first assess the representativeness of users on Reddit from each state of varied personality and culture. We ask,
% \vspace{0.1cm}
% {\indent\it RQ1. Which personality, culture, socioeconomic, and political attributes are associated with higher Reddit adoption rate by a state?}

\begin{enumerate}[label={}]
    \item\it RQ1. Which personality and cultural attributes are associated with higher Reddit adoption rate by a state?
\end{enumerate}

We observe that states with more restrictive cultural norms and are republican-leaning have lower Reddit adoption rate (less presence) than states with loose cultural norms and are democratic-leaning. Results here are consistent with prior work~\cite{duggan20136}.

Next, after controlling for each state's Reddit adoption rate  (presence on reddit), we focus on the circulation volume of news by states. The circulation volume of each state is of particular importance given that prior work demonstrates that repeated exposure to misinformation results in audience perceiving it to be more credibly~\cite{schwarz2020fake}. We also evaluate whether a state's personality and culture are significant indicators for the state's circulation and disproportionate circulation of true and false news on Reddit. Here, we include socioeconomic and political attributes of a states as additional control variables. Comparisons between the categories of variables can provide insights on which types of attributes are better indicators of news circulation than others. Specifically, we ask:
\begin{enumerate}[label={}]
    \item\it RQ2(a). Which states are outputting more reputable or non-reputable news? Are personality and cultural factors indicative of circulation? If so, are the results still significant even after we control for other attributes (socioeconomic, political, and platform factors)?
    \item\it RQ2(b). Which states have disproportionate output for misinformation? In other words, is a state's circulation volume of misinformation more (or less) than what's expected? Furthermore, are personality and cultural factors associated with this disproportionality?
\end{enumerate}

We observe that a state's news circulation volume is dominant a result of number of users present from that state. In fact, the number of users alone can explain 95\% ($R\approx 0.95$) of the variance we see in circulation volumes across the states. Interesting, the remaining residual can be explained by predominantly by personality and cultural factors. More specifically, the variance explained by personality and cultural factors is 50\% to 80\% of the variance explained by using all factors. In fact, the regression model using only psychological and cultural factors have a higher adjusted $R^2$ than models that exclusive use socioeconomic ($R^2\approx \{0.1, 0.25\}$) or political factors ($R^2\approx \{0.02, 0.2\}$). Next, focusing on disproportionate circulation, we observe that states rated high in {\it openness}(imaginative and spontaneous), have significantly higher output of reputable news than average, suggesting better informational return.

Finally, just as individuals with different personalities have distinct behaviors on social media~\cite{bachrach2012personality}, and that the ``winning personality" (e.g., optimistic and trusting) are more likely to be influential online than others~\cite{mohammadinejad2016employing}, a state's personality may also be associated with its influence on other states. That is to say, when a state shares a news article, is this article more likely to be propagated to other states resulting in news cascading due to the personalities and culture of the initial state? Furthermore, is a state's influence comparable for different news types? In addition, prior studies on Homophily have shown that states with similar characteristics have stronger social connections (or social tie)~\cite{boulianne2015social,kuchler2021jue}. For instance, related work by Bailey et al.~\cite{bailey2018social} demonstrates that users from similar states are more likely to be friends on Facebook. As such, we also examine whether states with similar personality and culture are more likely have a news propagation pathway (i.e., network edges)? we ask the following questions: 

\begin{enumerate}[label={}]
    \item\it RQ3(a). How frequent are news shared by a single state gets propagated to other states? If propagation exists, what's the most likely underlying network?
    \item\it RQ3(b). Which states are more influential than others within these networks? More importantly, is a state's personality and culture connected to its influence?
    \item\it RQ3(c). Does a state's influence vary for reputable news versus nonreputable news? That is, are certain states considerably influential when propagating reputable news, but less so when distributing misinformation (or vise versa).
    \item\it RQ3(d). Is social homophily an important indicator of contagion?
\end{enumerate}

We observe that geographical propagation of news articles is exceedingly rare on Reddit. Our analysis reveals that 86.7\% of all news articles are shared by only 1 or 2 redditors located in one of 50 states. Only 7.3\% or 209.7K of all reputable URLs were eventually posted by users from 5 or more distinct states. The numbers of URLs are 2.23K, 11.0K, 1.14K for {\it fake, lowcred, satire} news respectively, suggesting that contagion is even rarer for {\it satire} and {\it fake} articles. Additionally, cascading time on Reddit is much longer compared to Twitter or Facebook. For the URLs that were posted by at least 5 states, the average cascading time is more than a year (results are comparable irrespective of news types). Nevertheless, from the 209.7K reputable and low-credibily news sites that were posted by at least 10\% of the states, we infer the most likely network using the timestamps of the posts of each URL. We identify influential states from the two contagion networks: {\it lowcred} and {\it reputable}.  Focusing on a state's characteristics and its influence, we observe that {\it openness} and {\it extraversion} are both positively correlated with a state having higher influence on both networks. Further, states with high openness has higher influence when propagating traditional news than misinformation.  Finally, our homophily analysis shows that networks are disassortative. In other words, news is more likely to spread from one state to another if the pair of states are dissimilar from each other in personality and culture.

% prior studies on Homophily have shown that states with similar characteristics have stronger social connections (or social tie)~\cite{boulianne2015social,kuchler2021jue}. For instance, related work by Bailey et al.~\cite{bailey2018social} demonstrates that users from similar states are more likely to be friends on Facebook. As such, we also assess whether users from states with comparable social and cultural characteristics are more likely to communicate with each other on Reddit, and have a stronger tie. Moreover, we evaluate whether news articles can propagate from one state to others through these existing ties (contagion), and whether certain states have more influence and thus are more successful with news propagation than others. 

%######################################################################################################################################################################################################################################################################################################################################################################################################################
% Prior studies on misinformation~\cite{} demonstrates that false content in the United State is often politically driven~\cite{}. Further, the vast majority of fake news stories are conservative-leaning. Indeed, some scholars and pundits even attributed the outcome of the 2016 presidential election to the circulation and consumption of fake news~\cite{silverman2016here}. There have been many important studies focused on examining the overall circulation of misinformation online including i) the absolute volume of nonreputable news compared to reputable news, ii) the temporal trend of misinformation (i.e., do we see more circulation of misinformation overtime?), and iii) entities (i.e., individuals or news sites) who are most influential for circulating and propagating false content (contagion). Other researchers had sought out to understand an individual's attributes that are indicative of their likelihood of sharing misinformation online as well as their overall importance in the propagation of misinformation. As an example, literature demonstrates that conservatives' higher circulation and acceptance of misinformation may be associated with conservatives being more credulous to negative information.

% For our work, we expand the existing literature by centering our paper on understanding the geographical characteristics of misinformation. Indeed, the current political structure of the United States assures that a handful of battleground swing states alone can determine critical political outcomes. In fact, the winner of 2016 presidential election was chosen by 80K voters from 3 swing states. As such, in our paper, we first evaluate the circulation of reputable and nonreputable news across the individual states. For instance, is the circulation of false content higher than what's expected for swing states? Next, we explore the relationship between a state's news circulation volume and the state' psychological, cultural, socioeconomic, and political dimensions. To elaborate, we first categorize approximately 10K existing news websites into 4 types: fake, low-credibility, satire, and reputable. We then scrap Reddit's archival data and extract user comments containing URLs to these sites. We compute each state's overall circulation volume using redditors' estimated geographical location. Surprisingly, after controlling for each state's Reddit adoption rate, we observe that a state's psychological attributes are more indicative of the state's overall circulation of news as well as disproportionate circulation of news.

% Next, we examine whether certain states are more influential than others when distributing news. That is, whether news articles posted by certain states have more pathways to propagate to other states. Unlike social media platforms such as Twitter and Facebook where individual users can replicate and distribute news to their immediate network, Reddit is functionally an online forum, where many anonymous users interact under shared posts. Further, subreddits (sub-forums) are activity moderated by mods who generally discourages reposts (duplication of news articles). Our analysis reveals that 86.7\% of all news articles are shared by only 1 or 2 redditors. Only 7.3\% or 209.7K of all reputable URLs were eventually posted by 5 or more states. The numbers of URLs are 2.23K, 11.0K, 1.14K for {\it fake, lowcred, satire} news respectively. Additionally, for the URLs that were posted by at least 5 states, the average cascading time is more than a year (results are comparable irrespective of news types). In other words, our results confirm that news cascading is exceeding rare on Reddit especially for fake and satire news articles. Nevertheless, from the 209.7K reputable and low-credibily news sites that were posted by at least 10\% of the states, we extrapolated the most likely network using the timestamps of the posts of each URL. We identify influential states from the two 

%\comments{Others have focused on the consumption of misinformation [maybe add audience analysis]}
% (gentzkow paper). demonstrated that individuals in the United States, on average, only saw 1 or 2 stories~\cite{}

==> tables/basic_netinf_top.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Fri Jul 16 09:00:40 2021
\begin{table}[t]
\centering
\begin{tabular}{rllll}
  \hline
rank & traditional & lowcred & fake & satire \\ 
  \hline
  1 & TX & NY & IL & TX \\ 
    2 & WA & CA & MD & MN \\ 
    3 & CA & TX & MO & FL \\ 
    4 & NY & IL & CA & GA \\ 
    5 & OR & WA & VT & IL \\ 
    6 & MN & FL & FL & UT \\ 
    7 & MA & GA & TX & AL \\ 
    8 & FL & WI & OR & PA \\ 
    9 & IL & MN & CT & NM \\ 
   10 & OH & TN & WA & NY \\ 
   \hline
\end{tabular}
\end{table}


==> tables/circulation_models_ave.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Aug 12, 2021 - 09:43:06 PM
\begin{table}[!t] \centering \scriptsize
    \caption{Regression Results for Circulation Fraction. Here, the dependent variable was calculated as the average number of comments posted by users from a given state for each news type. We observed comparable results: personality and culture were strong indicators of circulation.} 
  \label{tab:circulation_ave} 
\begin{tabular}{@{\extracolsep{-5pt}}lp{2.2cm} p{2.2cm} p{2.2cm} p{2.2cm} p{2.2cm} p{2.2cm}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable: circulation fraction}} \\ 
\cline{2-7} 
 & reputable mod (personality and culture) & reputable mod (complete) & lowcred mod (personality and culture) & lowcred mod (complete) & fake mod (personality and culture) & fake mod (complete) \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 extraversion & 0.208$^{*}$ (0.123) &  & 0.013 (0.009) &  & 0.004$^{*}$ (0.002) &  \\ 
  agreeableness & 0.283$^{*}$ (0.143) & 0.239$^{**}$ (0.118) & 0.019$^{*}$ (0.010) & 0.021$^{**}$ (0.009) & 0.004$^{*}$ (0.002) & 0.005$^{**}$ (0.002) \\ 
  conscientiousness & $-$0.398$^{**}$ (0.153) & $-$0.349$^{***}$ (0.120) & $-$0.029$^{**}$ (0.011) & $-$0.024$^{**}$ (0.009) & $-$0.006$^{**}$ (0.003) & $-$0.004$^{*}$ (0.002) \\ 
  openness & 0.329$^{**}$ (0.133) &  & 0.018$^{*}$ (0.010) &  & 0.004$^{*}$ (0.002) & $-$0.003 (0.002) \\ 
  cultural\_tightness & $-$0.306$^{**}$ (0.136) & $-$0.344$^{***}$ (0.123) & $-$0.017 (0.010) & $-$0.019$^{**}$ (0.009) & $-$0.003 (0.002) & $-$0.006$^{**}$ (0.002) \\ 
  no\_highschool &  & 0.294$^{**}$ (0.122) &  & 0.032$^{***}$ (0.008) &  & 0.009$^{***}$ (0.002) \\ 
  population &  & 0.267$^{**}$ (0.122) &  &  &  &  \\ 
  gdp &  & 0.373$^{**}$ (0.160) &  & 0.032$^{***}$ (0.011) &  & 0.007$^{***}$ (0.002) \\ 
  density &  & $-$0.229$^{*}$ (0.124) &  & $-$0.016 (0.010) &  &  \\ 
  Constant & 2.676$^{***}$ (0.107) & 2.676$^{***}$ (0.085) & 0.194$^{***}$ (0.008) & 0.194$^{***}$ (0.007) & 0.042$^{***}$ (0.002) & 0.042$^{***}$ (0.001) \\ 
 \hline \\[-1.8ex] 
Observations & 48 & 48 & 48 & 48 & 48 & 48 \\ 
R$^{2}$ & 0.396 & 0.638 & 0.311 & 0.523 & 0.275 & 0.496 \\ 
Adjusted R$^{2}$ & 0.324 & 0.574 & 0.229 & 0.453 & 0.189 & 0.423 \\ 
Residual Std. Error & 0.740 (df = 42) & 0.587 (df = 40) & 0.054 (df = 42) & 0.045 (df = 41) & 0.012 (df = 42) & 0.010 (df = 41) \\ 
F Statistic & 5.515$^{***}$ (df = 5; 42) & 10.056$^{***}$ (df = 7; 40) & 3.797$^{***}$ (df = 5; 42) & 7.478$^{***}$ (df = 6; 41) & 3.187$^{**}$ (df = 5; 42) & 6.735$^{***}$ (df = 6; 41) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/circulation_models_nonpol.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, Jul 19, 2021 - 02:22:44 PM
% Requires LaTeX packages: dcolumn 
\begin{table}[t] \centering \scriptsize
  \caption{Regression Results for Circulation on Non-political Subreddits. Here, the {\it perc fitted} models only used personality and cultural explanatory variables. The {\it fitted} models used all explanatory variables. Personality and cultural factors alone explained a significant portion of the variance. Results here are consistent with prior observations.} 
  \label{tab:circulation_nonpol} 
\begin{tabular}{@{\extracolsep{-5pt}}lp{1.4cm} p{1.2cm} p{1.4cm} p{1.2cm} p{1.4cm} p{1.2cm} p{1.4cm} p{1.2cm}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{8}{c}{\textit{Dependent variable: circulation residual}} \\ 
\cline{2-9} 
 & {reputable mod (perc fitted)} & {reputable mod (fitted)} & {lowcred mod (perc fitted)} & {lowcred mod (fitted)} & {fake mod (perc fitted)} & {fake mod (fitted)} & {satire mod (perc fitted)} & {satire mod (fitted)} \\ 
\\[-1.8ex] & {(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)}\\ 
\hline \\[-1.8ex] 
Personality and Culture &&&&&&\\ 
 \hspace{0.3cm}agreeableness &  & 0.021 &  &  &  &  &  &  \\ 
  &  & (0.013) &  &  &  &  &  &  \\ 

 \hspace{0.3cm}conscientiousness & $-$0.052$^{***}$ & $-$0.046$^{***}$ & $-$0.046$^{***}$ & $-$0.047$^{***}$ & $-$0.076$^{***}$ & $-$0.051$^{***}$ & $-$0.047$^{**}$ &  \\ 
  & (0.016) & (0.013) & (0.013) & (0.012) & (0.017) & (0.017) & (0.019) &  \\  

 \hspace{0.3cm}extraversion &  &  &  &  & 0.026 &  &  &  \\ 
  &  &  &  &  & (0.018) &  &  &  \\ 
 
 \hspace{0.3cm}neuroticism & $-$0.020 &  &  &  &  &  &  & 0.023 \\ 
  & (0.014) &  &  &  &  &  &  & (0.015) \\ 
 
 \hspace{0.3cm}openness &  &  &  &  & 0.026 &  &  & $-$0.040$^{**}$ \\ 
  &  &  &  &  & (0.017) &  &  & (0.017) \\ 
 

 \hspace{0.3cm}cultural\_tightness & $-$0.031$^{**}$ & $-$0.030$^{**}$ & $-$0.024$^{*}$ &  &  &  & $-$0.055$^{***}$ & $-$0.047$^{**}$ \\ 
  & (0.013) & (0.014) & (0.013) &  &  &  & (0.019) & (0.019) \\ 
 

 Socioeconomic &&&&&&\\

 \hspace{0.3cm}density &  & $-$0.021 &  & $-$0.034$^{**}$ &  &  &  &  \\ 
  &  & (0.014) &  & (0.014) &  &  &  &  \\ 
 
 \hspace{0.3cm}no\_highschool &  & 0.023$^{**}$ &  & 0.023$^{**}$ &  & 0.021 &  &  \\ 
  &  & (0.011) &  & (0.011) &  & (0.016) &  &  \\ 
 
\hspace{0.3cm}gdp &  & 0.045$^{***}$ &  & 0.061$^{***}$ &  & 0.049$^{***}$ &  & 0.079$^{***}$ \\ 
  &  & (0.016) &  & (0.015) &  & (0.017) &  & (0.019) \\ 
  
 Constant & $-$0.007 & $-$0.007 & $-$0.003 & $-$0.003 & $-$0.001 & $-$0.001 & $-$0.009 & $-$0.009 \\ 
  & (0.010) & (0.009) & (0.012) & (0.010) & (0.016) & (0.015) & (0.016) & (0.015) \\ 
 
\hline \\[-1.8ex] 
Observations & 48 & 48 & 48 & 48 & 48 & 48 & 48 & 48 \\ 
R$^{2}$ & 0.485 & 0.598 & 0.369 & 0.519 & 0.334 & 0.408 & 0.387 & 0.532 \\ 
Adjusted R$^{2}$ & 0.450 & 0.539 & 0.341 & 0.474 & 0.288 & 0.368 & 0.359 & 0.489 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{8}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> tables/circulation_models_other.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Aug 12, 2021 - 09:39:48 PM
\begin{table}[!t] \centering \small
\caption{Regression Results for Circulation Using All Attributes Except for Personality and Culture. We saw that personality and cultural factors explained any additional 10\% to 20\% of the variance. As an example, the full model for reputable news using all variables had adjusted $R^2=0.45$. Here, we saw that the same model excluding personality and culture only had adjusted $R^2=0.338$ (a difference of approximately 0.11).}
  \label{tab:circulation_partial_other} 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable: circulation}} \\ 
\cline{2-4} 
 & reputable & lowcred & fake \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 no\_highschool &  & 0.033 (0.022) &  \\ 
  gdp & 0.062$^{***}$ (0.017) & 0.072$^{***}$ (0.022) & 0.049$^{***}$ (0.016) \\ 
  minority &  & $-$0.031 (0.022) &  \\ 
  density & $-$0.038$^{**}$ (0.017) & $-$0.033 (0.020) &  \\ 
  republican & $-$0.033$^{**}$ (0.016) & $-$0.025 (0.019) &  \\ 
  Constant & $-$0.006 (0.012) & $-$0.002 (0.014) & 0.001 (0.016) \\ 
 \hline \\[-1.8ex] 
Observations & 48 & 48 & 48 \\ 
R$^{2}$ & 0.380 & 0.313 & 0.170 \\ 
Adjusted R$^{2}$ & 0.338 & 0.231 & 0.152 \\ 
Residual Std. Error & 0.084 (df = 44) & 0.096 (df = 42) & 0.108 (df = 46) \\ 
F Statistic & 9.003$^{***}$ (df = 3; 44) & 3.831$^{***}$ (df = 5; 42) & 9.451$^{***}$ (df = 1; 46) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/circulation_models_pol.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, Jul 19, 2021 - 02:22:44 PM
% Requires LaTeX packages: dcolumn 
\begin{table}[!t] \centering \scriptsize
  \caption{Regression Results for Circulation on Political Subreddits. Here, the {\it perc fitted} models only used personality and cultural explanatory variables. The {\it fitted} models used all explanatory variables. Personality and cultural factors alone explained a significant portion of the variance. Results here are consistent with prior observations.} 
  \label{tab:circulation_pol} 
\begin{tabular}{@{\extracolsep{-5pt}}lp{1.4cm} p{1.2cm} p{1.4cm} p{1.2cm} p{1.4cm} p{1.2cm} p{1.4cm} p{1.2cm}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{8}{c}{\textit{Dependent variable: circulation residual}} \\ 
\cline{2-9} 
 & {reputable mod (perc fitted)} & {reputable mod (fitted)} & {lowcred mod (perc fitted)} & {lowcred mod (fitted)} & {fake mod (perc fitted)} & {fake mod (fitted)} & {satire mod (perc fitted)} & {satire mod (fitted)} \\ 
\\[-1.8ex] & {(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)}\\ 
\hline \\[-1.8ex] 
Personality and Culture &&&&&&\\ 
 \hspace{0.3cm}agreeableness & 0.028 & 0.040$^{*}$ & 0.031 & 0.043$^{*}$ &  & 0.043$^{*}$ &  & 0.046$^{*}$ \\ 
  & (0.018) & (0.021) & (0.020) & (0.022) &  & (0.023) &  & (0.027) \\ 
 
  \hspace{0.3cm}conscientiousness & $-$0.060$^{***}$ & $-$0.043 & $-$0.050$^{**}$ &  & $-$0.032$^{*}$ & $-$0.032 & $-$0.047$^{*}$ & $-$0.066$^{**}$ \\ 
  & (0.019) & (0.026) & (0.021) &  & (0.018) & (0.024) & (0.024) & (0.027) \\
  \hspace{0.3cm}neuroticism &  & 0.037 &  & 0.059$^{***}$ &  &  &  &  \\ 
  &  & (0.026) &  & (0.021) &  &  &  &  \\ 
   \hspace{0.3cm}openness &  &  &  &  &  & $-$0.044$^{*}$ &  &  \\ 
  &  &  &  &  &  & (0.026) &  &  \\ 
  \hspace{0.3cm}cultural\_tightness & $-$0.034$^{*}$ & $-$0.036 & $-$0.031 & $-$0.037 &  & $-$0.051$^{*}$ & $-$0.051$^{**}$ & $-$0.067$^{**}$ \\ 
  & (0.017) & (0.022) & (0.019) & (0.023) &  & (0.027) & (0.024) & (0.026) \\ 
Socioeconomic &&&&&&\\
  \hspace{0.3cm}density &  & $-$0.041 &  & $-$0.046$^{*}$ &  &  &  & 0.034 \\ 
  &  & (0.025) &  & (0.026) &  &  &  & (0.023) \\ 

  \hspace{0.3cm}gdp &  & 0.048 &  & 0.082$^{***}$ &  & 0.040$^{*}$ &  &  \\ 
  &  & (0.030) &  & (0.029) &  & (0.023) &  &  \\ 
 
  \hspace{0.3cm}minority &  & 0.028 &  &  &  &  &  &  \\ 
  &  & (0.019) &  &  &  &  &  &  \\ 

  \hspace{0.3cm}no\_highschool &  &  &  & 0.032$^{*}$ &  & 0.063$^{**}$ &  &  \\ 
  &  &  &  & (0.018) &  & (0.024) &  &  \\ 
 
Political &&&&&&\\
  \hspace{0.3cm}political &  &  &  &  &  &  &  & $-$0.035 \\ 
  &  &  &  &  &  &  &  & (0.024) \\ 
 Constant & $-$0.005 & $-$0.005 & $-$0.002 & $-$0.002 & 0.001 & 0.001 & $-$0.006 & $-$0.006 \\ 
  & (0.015) & (0.014) & (0.017) & (0.016) & (0.018) & (0.017) & (0.021) & (0.020) \\ 
 
\hline \\[-1.8ex] 
Observations & 48 & 48 & 48 & 48 & 48 & 48 & 48 & 48 \\ 
R$^{2}$ & 0.336 & 0.424 & 0.219 & 0.331 & 0.061 & 0.278 & 0.268 & 0.359 \\ 
Adjusted R$^{2}$ & 0.291 & 0.323 & 0.166 & 0.234 & 0.041 & 0.172 & 0.235 & 0.283 \\
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{8}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> tables/circulation_models_political.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Aug 12, 2021 - 09:38:48 PM
\begin{table}[!t] \centering \small
\caption{Regression Results for Circulation Using Only Political Attributes. We saw that Republican-leaning and politically disengaged states had lower-than-expected circulation. More importantly, we also observed that the variance explained by political attributes was much lower than the variance explained by personality and cultural factors (see Table 3 in the main text).} 
  \label{tab:circulation_partial_pol}  
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable: circulation}} \\ 
\cline{2-4} 
 & reputable & lowcred & fake \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 republican & $-$0.043$^{***}$ (0.013) & $-$0.040$^{**}$ (0.015) & $-$0.032$^{*}$ (0.017) \\ 
  political & 0.026$^{*}$ (0.013) &  &  \\ 
  Constant & $-$0.006 (0.013) & $-$0.002 (0.015) & 0.001 (0.016) \\ 
 \hline \\[-1.8ex] 
Observations & 48 & 48 & 48 \\ 
R$^{2}$ & 0.246 & 0.131 & 0.075 \\ 
Adjusted R$^{2}$ & 0.213 & 0.112 & 0.055 \\ 
Residual Std. Error & 0.092 (df = 45) & 0.103 (df = 46) & 0.114 (df = 46) \\ 
F Statistic & 7.342$^{***}$ (df = 2; 45) & 6.939$^{**}$ (df = 1; 46) & 3.754$^{*}$ (df = 1; 46) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/circulation_models_satire.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Aug 12, 2021 - 10:39:43 PM
\begin{table}[!t] \centering \small
\caption{Circulation of Satirical News. We again saw that that personality and cultural factors (specifically, {\it conscientiousness} and {\it cultural tightness}) alone explained a considerable portion of the variance.} 
  \label{tab:circulation_satire} 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable: circulation}} \\ 
\cline{2-5} 
 & personality and culture & socioeconomic & political & complete \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 conscientiousness & $-$0.047$^{**}$ (0.019) &  &  &  \\ 
  agreeableness &  &  &  & 0.033 (0.021) \\ 
  neuroticism &  &  &  & 0.048$^{**}$ (0.019) \\ 
  cultural\_tightness & $-$0.054$^{***}$ (0.019) &  &  & $-$0.050$^{**}$ (0.021) \\ 
  gdp &  & 0.091$^{***}$ (0.017) &  & 0.067$^{***}$ (0.021) \\ 
  minority &  & $-$0.042$^{**}$ (0.017) &  &  \\ 
  republican &  &  & $-$0.051$^{**}$ (0.019) &  \\ 
  political &  &  & 0.035$^{*}$ (0.019) &  \\ 
  Constant & $-$0.008 (0.017) & $-$0.008 (0.016) & $-$0.008 (0.019) & $-$0.008 (0.016) \\ 
 \hline \\[-1.8ex] 
Observations & 48 & 48 & 48 & 48 \\ 
R$^{2}$ & 0.370 & 0.398 & 0.193 & 0.455 \\ 
Adjusted R$^{2}$ & 0.342 & 0.372 & 0.157 & 0.405 \\ 
Residual Std. Error & 0.116 (df = 45) & 0.113 (df = 45) & 0.131 (df = 45) & 0.110 (df = 43) \\ 
F Statistic & 13.229$^{***}$ (df = 2; 45) & 14.897$^{***}$ (df = 2; 45) & 5.369$^{***}$ (df = 2; 45) & 8.984$^{***}$ (df = 4; 43) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/circulation_models_socio.tex <==
\begin{table}[!t] \centering \small
\caption{Regression Results for Circulation Using Only Socioeconomic Attributes. We saw that states with a higher average income had higher-than-expected circulation for all news types. More importantly, the variance explained by socioeconomic conditions was comparable or slightly lower than the variance explained by personality and cultural factors (see Table 3).}
  \label{tab:circulation_partial_socio} 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable: circulation}} \\ 
\cline{2-4} 
 & reputable & lowcred & fake \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 no\_highschool &  & 0.035 (0.022) &  \\ 
  gdp & 0.071$^{***}$ (0.017) & 0.066$^{***}$ (0.017) & 0.049$^{***}$ (0.016) \\ 
  density & $-$0.024 (0.017) &  &  \\ 
  minority &  & $-$0.034 (0.022) &  \\ 
  Constant & $-$0.006 (0.013) & $-$0.002 (0.014) & 0.001 (0.016) \\ 
 \hline \\[-1.8ex] 
Observations & 48 & 48 & 48 \\ 
R$^{2}$ & 0.319 & 0.256 & 0.170 \\ 
Adjusted R$^{2}$ & 0.289 & 0.206 & 0.152 \\ 
Residual Std. Error & 0.087 (df = 45) & 0.097 (df = 44) & 0.108 (df = 46) \\ 
F Statistic & 10.530$^{***}$ (df = 2; 45) & 5.053$^{***}$ (df = 3; 44) & 9.451$^{***}$ (df = 1; 46) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/contagion_models.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Jul 20, 2021 - 08:52:07 AM
% Requires LaTeX packages: dcolumn 
\begin{table}[t] \centering \scriptsize
  \caption{Regression results for {\it pagerank} generated using the 10\% threshold networks (results are comparable for 20\% threshold networks). A higher {\it pagerank} suggests that a state has more influence when diffusing news. Here, the {\it perc fitted} models only use perchological and cultural explanatory variables. The {\it fitted} models use all explanatory variables. Again, we see that personality and cultural factors are significant in predicting a state's pagerank (influence.)} 
  \label{tab:pagerank} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & \multicolumn{4}{c}{pagerank} \\ 
 & \multicolumn{1}{c}{traditional (perc fitted)} & \multicolumn{1}{c}{traditional (fitted)} & \multicolumn{1}{c}{lowcred (perc fitted)} & \multicolumn{1}{c}{lowcred (fitted)} \\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)}\\ 
\hline \\[-1.8ex] 
  extraversion & 0.097^{**}$ $(0.044) &  & 0.140^{***}$ $(0.044) &  \\ 
  agreeableness &  & 0.068^{*}$ $(0.036) &  & 0.061$ $(0.038) \\ 
  openness & 0.206^{***}$ $(0.046) & 0.117^{***}$ $(0.037) & 0.119^{**}$ $(0.049) &  \\ 
  cultural\_tightness &  &  & -0.087^{*}$ $(0.046) &  \\ 
  population &  & 0.165^{***}$ $(0.034) &  & 0.180^{***}$ $(0.034) \\ 
  gdp &  & 0.220^{***}$ $(0.065) &  & 0.110$ $(0.074) \\ 
  republican &  &  &  & -0.094^{**}$ $(0.041) \\ 
  political &  &  &  & 0.062^{*}$ $(0.032) \\ 
  swing\_state &  & 0.073^{**}$ $(0.029) &  & 0.051$ $(0.032) \\ 
  Constant & 0.359^{***}$ $(0.041) & 0.371^{***}$ $(0.029) & 0.472^{***}$ $(0.040) & 0.474^{***}$ $(0.031) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.315} & \multicolumn{1}{c}{0.710} & \multicolumn{1}{c}{0.292} & \multicolumn{1}{c}{0.631} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.285} & \multicolumn{1}{c}{0.676} & \multicolumn{1}{c}{0.244} & \multicolumn{1}{c}{0.577} \\ 
Residual Std. Error & \multicolumn{1}{c}{0.283 (df = 45)} & \multicolumn{1}{c}{0.190 (df = 42)} & \multicolumn{1}{c}{0.278 (df = 44)} & \multicolumn{1}{c}{0.208 (df = 41)} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/pagerank_diff_models.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Jul 20, 2021 - 08:14:41 AM
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering \scriptsize
  \caption{Regression results for {\it pagerank differential}, which is computed as subtracting states' pagerank percentile rank in the {\it traditional} news network by the corresponding pagerank percentile rank in the {\it lowcred} news network. A positive {\it pagerank differential} suggests that a state has more influence when diffusing traditional news. Here, the {\it psyc fitted} models only use psychological and cultural explanatory variables. The {\it fitted} models use all explanatory variables. We see that psychological and cultural factors are, in fact, the most important explanatory variables.}
  \label{tab:pagerank_diff}
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable: {\it pagerank differential}}} \\ 
\cline{2-5} 
\\[-1.8ex] 
 & \multicolumn{1}{c}{10\% threshold (psyc fitted)} & \multicolumn{1}{c}{10\% threshold (fitted)} & \multicolumn{1}{c}{20\% threshold (psyc fitted)} & \multicolumn{1}{c}{20\% threshold (fitted)} \\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)}\\ 
\hline \\[-1.8ex] 
 openness & 0.061^{**}$ $(0.026) & 0.079^{***}$ $(0.027) & 0.070^{**}$ $(0.028) & 0.091^{***}$ $(0.030) \\ 
  density &  & -0.241$ $(0.145) &  & -0.287^{*}$ $(0.158) \\ 
  Constant & -0.113^{***}$ $(0.023) & -0.146^{***}$ $(0.030) & -0.041$ $(0.026) & -0.081^{**}$ $(0.033) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.110} & \multicolumn{1}{c}{0.161} & \multicolumn{1}{c}{0.120} & \multicolumn{1}{c}{0.180} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.090} & \multicolumn{1}{c}{0.124} & \multicolumn{1}{c}{0.101} & \multicolumn{1}{c}{0.144} \\ 
Residual Std. Error & \multicolumn{1}{c}{0.162 (df = 46)} & \multicolumn{1}{c}{0.159 (df = 45)} & \multicolumn{1}{c}{0.177 (df = 46)} & \multicolumn{1}{c}{0.173 (df = 45)} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/pol_frac_models.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, Jul 26, 2021 - 11:41:12 AM
\begin{table}[!htbp] \centering \scriptsize
  \caption{The dependent variable is the fraction of news that were shared on political subreddits for each type of news. As an example, 73.5\% of all {\it fake} news posted by Alabama users were shared on political subreddits. Whereas, only 55\% of all {\it fake} news posted by Arizona were shared on political subreddits. On average, 44.2\% reputable news are shared on political subreddits compared to 67.3\% for fake news, and 58\% for low-credibility news, and 39\% for satire news. We observe that states ranked higher on {\it openness} tend to share less news (irrespective of news types) on political subreddits.} 
  \label{} 
\begin{tabular}{lp{1.2cm}p{1.4cm}p{1.6cm}p{1.6cm}p{1.4cm}p{1.4cm}p{1.4cm}p{1.4cm}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{8}{c}{\textit{Dependent variable:}} \\ 
\\[-1.8ex]\hline\cline{2-9} 
 & all news (pysc fitted) & all news (fitted) & lowcred+reputable news (psyc fitted) & lowcred+reputable news (fitted) & fake+reputable news  (psyc fitted) & fake+reputable news (fitted) & satire+reputable news  (psyc fitted) & satire+reputable news (fitted) \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
\hline \\[-1.8ex] 
 extraversion &  & $-$0.008 &  &  &  &  &  & $-$0.017$^{**}$ \\ 
  &  & (0.005) &  &  &  &  &  & (0.007) \\ 

 openness &  & $-$0.018$^{***}$ &  & $-$0.020$^{***}$ & $-$0.014 & $-$0.020$^{*}$ & 0.020$^{**}$ &  \\ 
  &  & (0.006) &  & (0.008) & (0.010) & (0.010) & (0.009) &  \\ 

 population &  & 0.012$^{*}$ &  & 0.010 &  &  &  &  \\ 
  &  & (0.006) &  & (0.007) &  &  &  &  \\ 

 gdp &  & $-$0.010$^{**}$ &  & $-$0.014$^{**}$ &  & $-$0.016 &  &  \\ 
  &  & (0.005) &  & (0.006) &  & (0.010) &  &  \\ 

 republican &  & $-$0.016$^{**}$ &  & $-$0.015$^{**}$ &  &  &  &  \\ 
  &  & (0.006) &  & (0.007) &  &  &  &  \\ 

 political &  &  &  &  &  & $-$0.015 &  &  \\ 
  &  &  &  &  &  & (0.009) &  &  \\ 

 cultural\_tightness &  &  &  &  & $-$0.016 & $-$0.019$^{*}$ &  &  \\ 
  &  &  &  &  & (0.011) & (0.011) &  &  \\ 

 agreeableness &  &  & 0.015$^{**}$ &  & 0.019 & 0.015 & 0.021$^{**}$ &  \\ 
  &  &  & (0.007) &  & (0.012) & (0.010) & (0.010) &  \\ 

 conscientiousness &  &  &  &  & 0.023$^{*}$ &  &  &  \\ 
  &  &  &  &  & (0.013) &  &  &  \\ 

 neuroticism &  &  & 0.009 &  & 0.020$^{*}$ &  & 0.022$^{**}$ &  \\ 
  &  &  & (0.007) &  & (0.012) &  & (0.009) &  \\ 

 no\_highschool &  &  &  &  &  &  &  & 0.038$^{***}$ \\ 
  &  &  &  &  &  &  &  & (0.009) \\ 

 minority &  &  &  &  &  &  &  & $-$0.026$^{***}$ \\ 
  &  &  &  &  &  &  &  & (0.009) \\ 

 density &  &  &  &  &  &  &  & 0.018$^{**}$ \\ 
  &  &  &  &  &  &  &  & (0.008) \\ 

 Constant & 0.444$^{***}$ & 0.444$^{***}$ & 0.583$^{***}$ & 0.583$^{***}$ & 0.673$^{***}$ & 0.673$^{***}$ & 0.392$^{***}$ & 0.392$^{***}$ \\ 
  & (0.005) & (0.005) & (0.006) & (0.006) & (0.008) & (0.008) & (0.008) & (0.007) \\ 

\hline \\[-1.8ex] 
Observations & 48 & 48 & 48 & 48 & 48 & 48 & 48 & 48 \\ 
R$^{2}$ & 0.000 & 0.235 & 0.099 & 0.190 & 0.233 & 0.261 & 0.154 & 0.336 \\ 
Adjusted R$^{2}$ & 0.000 & 0.144 & 0.059 & 0.115 & 0.141 & 0.173 & 0.096 & 0.274 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{8}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/roi_models.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Jul 20, 2021 - 07:44:22 AM
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering \scriptsize
  \caption{Return of Investment (ROI) Regression Results. Here, the {\it psyc fitted} models only use psychological and cultural explanatory variables. The {\it fitted} models use all explanatory variables. We see that the variance explained by psychological and cultural factors is approximately half of the variance explained by using all factors for all news except {\it satire}.} 
  \label{tab:roi} 
\begin{tabular}{lp{0.8cm}p{0.8cm}p{1.3cm}p{1.3cm}p{1.1cm}p{1cm}p{1.2cm}p{1cm}}
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{8}{c}{\textit{Dependent variable: ROI}} \\ 
\cline{2-9} 
 & {all news (pysc fitted)} & {all news (fitted)} & {lowcred+ reputable news (psyc fitted)} & {lowcred+ reputable news (fitted)} & {fake+ reputable news (psyc fitted)} & {fake+ reputable news (fitted)} & {satire+ reputable news (psyc fitted)} & {satire+ reputable news (fitted)} \\ 
\\[-1.8ex] & {(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)}\\ 
\hline \\[-1.8ex] 
openness & 0.313$^{*}$ & 0.357$^{**}$ & 0.267$^{**}$ &  &  & 0.075$^{*}$ &  &  \\ 
  & (0.163) & (0.161) & (0.129) &  &  & (0.044) &  &  \\ 

 no\_highschool &  & $-$0.275$^{*}$ &  &  &  & $-$0.096$^{**}$ &  &  \\ 
  &  & (0.148) &  &  &  & (0.040) &  &  \\ 

 neuroticism &  &  &  & $-$0.222$^{*}$ &  &  &  &  \\ 
  &  &  &  & (0.127) &  &  &  &  \\ 

 republican &  &  &  & $-$0.311$^{**}$ &  &  &  &  \\ 
  &  &  &  & (0.144) &  &  &  &  \\ 

 political &  &  &  & 0.165 &  &  &  &  \\ 
  &  &  &  & (0.120) &  &  &  &  \\ 

 cultural\_tightness &  &  &  &  & $-$0.078$^{*}$ &  & 0.027$^{*}$ &  \\ 
  &  &  &  &  & (0.041) &  & (0.016) &  \\ 

 minority &  &  &  &  &  &  &  & 0.051$^{***}$ \\ 
  &  &  &  &  &  &  &  & (0.016) \\ 

 density &  &  &  &  &  &  &  & $-$0.353$^{***}$ \\ 
  &  &  &  &  &  &  &  & (0.082) \\ 

 Constant & $-$0.286$^{*}$ & $-$0.279$^{*}$ & $-$0.243$^{**}$ & $-$0.231$^{*}$ & $-$0.055 & $-$0.049 & $-$0.003 & $-$0.049$^{***}$ \\ 
  & (0.150) & (0.146) & (0.118) & (0.115) & (0.041) & (0.040) & (0.016) & (0.018) \\ 

\hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.074} & \multicolumn{1}{c}{0.140} & \multicolumn{1}{c}{0.085} & \multicolumn{1}{c}{0.177} & \multicolumn{1}{c}{0.073} & \multicolumn{1}{c}{0.144} & \multicolumn{1}{c}{0.060} & \multicolumn{1}{c}{0.329} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.054} & \multicolumn{1}{c}{0.102} & \multicolumn{1}{c}{0.065} & \multicolumn{1}{c}{0.120} & \multicolumn{1}{c}{0.053} & \multicolumn{1}{c}{0.106} & \multicolumn{1}{c}{0.039} & \multicolumn{1}{c}{0.299} \\ 
Residual Std. Error & \multicolumn{1}{c}{1.036 (df = 46)} & \multicolumn{1}{c}{1.010 (df = 45)} & \multicolumn{1}{c}{0.818 (df = 46)} & \multicolumn{1}{c}{0.794 (df = 44)} & \multicolumn{1}{c}{0.282 (df = 46)} & \multicolumn{1}{c}{0.274 (df = 45)} & \multicolumn{1}{c}{0.109 (df = 46)} & \multicolumn{1}{c}{0.093 (df = 45)} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{8}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/roi_models_v2.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, Jul 26, 2021 - 10:41:21 AM
\begin{table}[!htbp] \centering \scriptsize
  \caption{Return of Investment (ROI) differentiated by political and non-political subreddits. That is, does a state post more reputable news than what's expected on political subreddits(positive ROI)? What about news circulation on non-political subreddits. Results here suggests that states rated high in {\it openness} have higher ROI for political subreddits, and {\it republican-leaning} and less educated states have lower ROI. \todo{the adj r2 are close to zero}} 
  \label{} 
\begin{tabular}{lp{3cm}p{3cm}p{3cm}p{3cm}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & \multicolumn{4}{c}{roi} \\ 
 & all news on non-political subreddits (pysc fitted) & all news on non-political subreddits (fitted) & all news on political subreddits (pysc fitted) & all news on political subreddits (fitted) \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 conscientiousness & 0.198$^{**}$ &  &  &  \\ 
  & (0.098) &  &  &  \\ 

 cultural\_tightness & $-$0.231$^{**}$ &  &  & 0.856$^{*}$ \\ 
  & (0.098) &  &  & (0.477) \\ 

 neuroticism &  & $-$0.224$^{**}$ &  &  \\ 
  &  & (0.092) &  &  \\ 

 no\_highschool &  & $-$0.137 &  & $-$1.017$^{**}$ \\ 
  &  & (0.098) &  & (0.420) \\ 

 gdp &  & $-$0.185$^{*}$ &  &  \\ 
  &  & (0.104) &  &  \\ 

 density &  &  &  & $-$0.571$^{*}$ \\ 
  &  &  &  & (0.325) \\ 

 republican &  & $-$0.196$^{*}$ &  & $-$0.761$^{**}$ \\ 
  &  & (0.098) &  & (0.376) \\ 

 openness &  &  & 0.507$^{*}$ & 0.819$^{**}$ \\ 
  &  &  & (0.256) & (0.361) \\ 

 Constant & $-$0.129 & $-$0.129 & $-$0.588$^{**}$ & $-$0.588$^{**}$ \\ 
  & (0.085) & (0.085) & (0.253) & (0.242) \\ 

\hline \\[-1.8ex] 
Observations & 48 & 48 & 48 & 48 \\ 
R$^{2}$ & 0.129 & 0.178 & 0.079 & 0.235 \\ 
Adjusted R$^{2}$ & 0.090 & 0.101 & 0.059 & 0.144 \\ 
Residual Std. Error & 0.590 (df = 45) & 0.586 (df = 43) & 1.755 (df = 46) & 1.674 (df = 42) \\ 
F Statistic & 3.325$^{**}$ (df = 2; 45) & 2.320$^{*}$ (df = 4; 43) & 3.930$^{*}$ (df = 1; 46) & 2.580$^{**}$ (df = 5; 42) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table}

==> tables/simpson_models.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Jul 20, 2021 - 11:00:47 AM
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering \scriptsize
  \caption{Simpson's Index Regression Results. Here, we compute simpson index for each state using the distribution of news posts across different subreddits. A higher simpson index (value between $[0, 1]$) indicates a more diverse audience. Here, the {\it psyc fitted} models only use psychological and cultural explanatory variables. The {\it fitted} models use all explanatory variables. We see that psychological and cultural factors include {\it agreeableness} and {\it conscientiousness} are associated with less diversity in audience.}
  \label{tab:simpson} 
\begin{tabular}{lp{1.2cm}p{1.2cm}p{1.3cm}p{1.3cm}p{1cm}p{1cm}p{1cm}p{1cm}}
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{8}{c}{\textit{Dependent variable: Simpson's Index}} \\ 
\cline{2-9} 
 & {traditional mod (psyc fitted)} & {traditional mod (fitted)} & {lowcred mod (psyc fitted)} & {lowcred mod (fitted)} & {fake mod (psyc fitted)} & {fake mod (fitted)} & {satire mod (psyc fitted)} & {satire mod (fitted)} \\ 
\\[-1.8ex] & {(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)}\\ 
\hline \\[-1.8ex] 
 agreeableness & -0.002^{**} & -0.002^{***} & -0.002 & -0.003^{*} &  &  &  &  \\ 
  & (0.001) & (0.001) & (0.001) & (0.001) &  &  &  &  \\ 

 neuroticism & -0.001^{*} &  &  &  &  &  &  &  \\ 
  & (0.001) &  &  &  &  &  &  &  \\ 

 conscientiousness &  &  &  &  & -0.007^{*} & -0.008^{*} &  &  \\ 
  &  &  &  &  & (0.004) & (0.004) &  &  \\ 

 extraversion &  &  &  &  &  &  & 0.004^{**} & 0.003^{*} \\ 
  &  &  &  &  &  &  & (0.002) & (0.002) \\ 

 openness & -0.001 &  &  &  & 0.007 & 0.007 & 0.003^{*} &  \\ 
  & (0.001) &  &  &  & (0.004) & (0.005) & (0.002) &  \\ 

 cultural\_tightness & 0.001 &  &  &  &  &  &  & 0.003 \\ 
  & (0.001) &  &  &  &  &  &  & (0.002) \\ 


 gdp &  &  &  & 0.004 &  &  &  &  \\ 
  &  &  &  & (0.003) &  &  &  &  \\ 

 density &  &  &  & -0.016^{**} &  & -0.052^{**} &  & -0.022^{**} \\ 
  &  &  &  & (0.007) &  & (0.025) &  & (0.010) \\ 

no\_highschool &  &  &  &  &  & -0.006 &  &  \\ 
  &  &  &  &  &  & (0.004) &  &  \\ 

 population &  & 0.001^{**} &  &  &  & 0.008^{*} &  & 0.004^{***} \\ 
  &  & (0.0005) &  &  &  & (0.004) &  & (0.002) \\ 

 republican &  & 0.003^{***} &  &  &  &  &  & -0.009^{***} \\ 
  &  & (0.001) &  &  &  &  &  & (0.002) \\ 

 political &  &  &  &  &  &  &  & 0.003^{*} \\ 
  &  &  &  &  &  &  &  & (0.002) \\ 

 Constant & 0.976^{***} & 0.975^{***} & 0.966^{***} & 0.965^{***} & 0.940^{***} & 0.932^{***} & 0.963^{***} & 0.961^{***} \\ 
  & (0.001) & (0.0005) & (0.001) & (0.001) & (0.004) & (0.005) & (0.002) & (0.002) \\ 

\hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{48} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.152} & \multicolumn{1}{c}{0.363} & \multicolumn{1}{c}{0.051} & \multicolumn{1}{c}{0.157} & \multicolumn{1}{c}{0.123} & \multicolumn{1}{c}{0.268} & \multicolumn{1}{c}{0.124} & \multicolumn{1}{c}{0.468} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.073} & \multicolumn{1}{c}{0.320} & \multicolumn{1}{c}{0.031} & \multicolumn{1}{c}{0.099} & \multicolumn{1}{c}{0.084} & \multicolumn{1}{c}{0.181} & \multicolumn{1}{c}{0.085} & \multicolumn{1}{c}{0.391} \\ 
Residual Std. Error & \multicolumn{1}{c}{0.004 (df = 43)} & \multicolumn{1}{c}{0.003 (df = 44)} & \multicolumn{1}{c}{0.008 (df = 46)} & \multicolumn{1}{c}{0.007 (df = 44)} & \multicolumn{1}{c}{0.027 (df = 45)} & \multicolumn{1}{c}{0.025 (df = 42)} & \multicolumn{1}{c}{0.011 (df = 45)} & \multicolumn{1}{c}{0.009 (df = 41)} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{8}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 
